A Generalized Framework for Video Instance Segmentation

The handling of long videos with complex and occluded sequences has recently emerged as a new challenge in the video instance segmentation (VIS) community. However, existing methods have limitations in addressing this challenge. We argue that the biggest bottleneck in current approaches is the discrepancy between training and inference. To effectively bridge this gap, we propose a Generalized framework for VIS, namely GenVIS, that achieves state-of-the-art performance on challenging benchmarks without designing complicated architectures or requiring extra post-processing. The key contribution of GenVIS is the learning strategy, which includes a query-based training pipeline for sequential learning with a novel target label assignment. Additionally, we introduce a memory that effectively acquires information from previous states. Thanks to the new perspective, which focuses on building relationships between separate frames or clips, GenVIS can be flexibly executed in both online and semi-online manner. We evaluate our approach on popular VIS benchmarks, achieving state-of-the-art results on YouTube-VIS 2019/2021/2022 and Occluded VIS (OVIS). Notably, we greatly outperform the state-of-the-art on the long VIS benchmark (OVIS), improving 5.6 AP with ResNet-50 backbone. Code is available at https://github.com/miranheo/GenVIS.

==> algorithm/training.tex <==
\begin{table}%[H]
	\centering
% 	\begin{minipage}[t]{0.49\linewidth}
%     \caption{
%     %
%     PyTorch-style inference pseudo-code of VITA~\cite{VITA}.
%     % 
%     }
%     \label{alg:vita}
%     \begin{python}
% def vita(video):






%     feats = backbone(video)
%     fq, mf = mask2former(feats)

%     del feats
    
%     fq = object_encoder(fq)
    
%     vq = object_decoder(fq)
    
    
%     w = mask_head(vq)



%     # w.shape: (Nv x C)
%     # mf.shape: (C x H x W)
%     pred_mask = w @ mf

%     # Nv x (K+1)
%     pred_cls = cls_head(vq)

%     # Nv x T x H x W
%     pred_mask = torch.stack(
%         pred_mask, dim=1
%     )

%     return pred_cls, pred_mask
%     \end{python}
%     %\vspace{-9mm}
% 	\end{minipage}
% 	\hfill
	% \begin{minipage}[t]{0.49\linewidth}
    
    \begin{python}
def GenVIS(video):
    pred_cls, pred_mask, memory = [], [], []
    q = object_decoder.q
    
    for clip in video:
        feats  = backbone(clip)
        fq, mf = mask2former(feats)
    
        fq     = object_encoder(fq)
        q, p   = object_decoder(fq, q, memory)
        
        memory.append(p)
    
        w = mask_head(q)
        
        # w.shape: (Nq x C)
        # mf.shape: (Nf x C x H x W)
        pred_mask.append(w @ mf)
        pred_cls.append(cls_head(q))
        
    return pred_cls, pred_mask
    \end{python}
    \vspace{-4mm}
	% \end{minipage}
    \caption{
    %
    PyTorch-style inference pseudo-code of GenVIS.
    % \texttt{mf} denotes mask feature of Mask2Former.
    % The arguments of \texttt{object_decoder} are,
    % % 
    }
    \vspace{-5mm}
    \label{alg:genvis}
\end{table}


==> fig/clip_len.tex <==
\begin{table*}
	\begin{minipage}{0.33\linewidth}
    {
        \centering
        \resizebox{\linewidth}{!}
        {
            \begin{tabular}{c|ccccc}
            \toprule
            $N_{f}$  & AP        & AP$_{50}$     & AP$_{75}$     & AR$_{1}$      & AR$_{10}$ \\
            \midrule
            \midrule
            1            & 33.0 & 56.8 & 34.3 & 15.7 & 37.5 \\ 
            \textbf{3}   & \textbf{33.4} & \textbf{57.8} & \textbf{34.5} & \textbf{15.7} & \textbf{37.7}  \\
            5            & 31.3 & 56.0 & 32.8 & 15.3 & 35.9  \\
            7            & 29.7 & 51.4 & 30.7 & 14.6 & 34.0 \\
            \bottomrule
            \end{tabular}
        }
        \caption{
            ablation ovis validation R50 - Number of frames for a clip - 5 clips are used for training. 
        }
        \label{tab:clip_len}
    }
	\end{minipage}
	\hfill
	\begin{minipage}{0.58\linewidth}
    % \resizebox{\linewidth}{!}
    {
        \centering
        {
            \includegraphics[width=1\linewidth]{fig_img/clip_len_per_dataset_ver6.pdf}
        }
        \vspace{-3mm}
        \caption{
            Maximum number of frames that can be processed at once using a single Titan XP.
        }
        \label{fig:clip_len}
        }
	\end{minipage}
    % \hfill
\end{table*}

==> fig/criterion.tex <==
\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{fig_img/criterion2.pdf}
    %\vspace{-6mm}
    \caption{
    Unified detection and tracking label assignment.
    By adopting this simple ground-truth assignment strategy that resembles the inference pipeline, the accuracy on the VIS task can be significantly improved without any bells-and-whistles.
    }
    \label{fig:criterion}
\end{figure}


==> fig/supp_qualitative.tex <==
\begin{figure*}[t]
\begin{center}
\includegraphics[width=\linewidth]{fig_img/supp_qualitative.pdf}
\end{center}
\vspace{-3mm}
\caption{
Qualitative comparisons of our method, GenVIS, with the state-of-the-art methods: MinVIS~\cite{MinVIS} and VITA~\cite{VITA}.
% The videos on the left and right are from YouTube-VIS 2022~\cite{MaskTrackRCNN} and OVIS~\cite{OVIS-Dataset} datasets, respectively.
GenVIS shows impressive accuracy in these complicated scenes where the objects look similar crossing each other. Objects with the same identity are displayed in the same color.
}
%\vspace{-4mm}
\label{fig:qualitative_supp}
\end{figure*}

==> sections/1_introduction_backup.tex <==
\section{Introduction}
\label{sec:intro}
% Humans are unceasingly able to distinguish objects, and make high-level reasoning based on the recognition.
Video Instance Segmentation (VIS) is the task of simultaneously segmenting, identifying, and tracking all objects in videos, which is an essential task in computer vision.
It can be applied to various applications such as autonomous driving, robot vision, and video editing.
With the recent advent of datasets consists of long and complicated sequences, the community makes a further step to the real-world.
Previous studies address the problem with largely two paradigms according to the units the model processes at the inference stage: \emph{frame} and \emph{clip/video}.
%To enable machines to handle these fundamental problems, Video Instance Segmentation (VIS) has been proposed~\cite{MaskTrackRCNN}.
%From its definition of simultaneously segmenting, identifying, and tracking all objects in videos, VIS can be applied to various applications such as autonomous driving, robot vision, and video editing.
% Video Instance Segmentation (VIS) is the task of simultaneously segmenting, identifying, and tracking all objects in videos, which is an essential task for enabling machines to handle these underlying problems.
% Video Instance Segmentation (VIS) - simultaneously segmenting, identifying, and tracking all objects in videos - is an essential computer visiontask that enables machines to handle these underlying problems.
% \textcolor{red}{Thanks to its definition analogous to human basic cognitive abilities, 
% It also has the potential to serve as a primary observation for high-level understandings, such as interpretation of human-object interactions.

%have proposed various models with different units at the inference stage: \emph{frame} and \emph{clip/video}.
%To understand a video, existing studies tackle this problem by making models to take different scopes: frame, clip, and video.
%Existing studies tackle this problem by taking different scopes that the model uses to infer the entire video: frame, clip, and video.
Most online methods deploy frame-level predictions
%take the assumption based on the nature of physical world;
% \textcolor{red}{1) real-world is a continuous and endless data series over time;}
%objects with the same identity typically have similar appearances and positions between adjacent time steps.
benefitting from the advances in image-level detection models~\cite{FCOS, SOLOv1, QueryInst, DETR, Deformable-DETR, Mask2Former} (\cref{fig:teaser} (a)).
Thanks to the video length-agnostic nature, recent works~\cite{MinVIS, IDOL} show its effectiveness in long videos.
However, existing approaches have relied heavily on hand-crafted algorithms in post-processing.
%since they focus on how to connect given frame-level detections.
% to achieve high performance, complex matching algorithms incorporated with handcrafted design are required in the post processing.
% However, they still have limitations on highly occluded or blurry objects, and require post association
% However, the inherent structures that are vulnerable to leveraging temporal information show limitations on highly occluded or blurry objects and \fix{inevitably lead to post-association}.

% %------------------------------
% \input{fig/teaser}
% %------------------------------


% 더 높은 성능을 위해 per-clip & offline이 제시되었다.
% per-clip은 비디오를 작은 단위로 쪼개고 ㄷ이를 이어붙이는 방법이 때문에 핸드 크래프티드 알고리즘이 필요하고, ㅇ그에 반해 offline은 전체 비디오를 한번ㅇ에 처리하여 이러한 알고리ㅂ즘을 생략할 수 있었다.
% 그러나 굉장히 긴 비디오를 처리해야하는 경우 offline도 비디오를 결국 gpu가 처리할 수 있는 단위로 쪼개야하고, 결국 clip의 길이가 매우 긴 per-clip방법으로 해석될 수 있다: 핸드 크래프티드 ㅇ알고리즘으로 스팃칭을 해야한다.

%On the other hand, the methods of taking multiple frames have been introduced (\cref{fig:teaser} (b)).
%Early study~\cite{MaskProp} proposes \emph{per-clip} approach that focuses on aggregating information from neighboring frames.
%Since it associates adjacent clips by using mask IoU of overlapped frames,  relies on heuristics.
On the other hand, \emph{video-in \& video-out} paradigm based on Transformer~\cite{Transformer} eliminates post-processing by taking the entire video as input and predict instance-wise mask trajectories in a single forward-pass~\cite{VisTR, IFC, Mask2Former-VIS, TeViT, SeqFormer, VITA} (\cref{fig:teaser} (b)).
% On the other hand, Transformer-based~\cite{Transformer} \emph{video-in \& video-out} paradigm~\cite{VisTR, IFC, Mask2Former-VIS, TeViT, SeqFormer, VITA} architectures take the entire video as input and predict instance-wise mask trajectories in a single forward-pass for a better accuracy.
% The benefits of such architecture are two folds:
% 1) it is robust against occlusion and motion blur by aggregating information from neighboring frames;
% One of the benefits of such architecture is that it removes the boundaries between training and inference in terms of association; model infers in exactly the same way as learned.
% Such architectures show robust performance against occlusion and motion blur by aggregating information from neighboring frames.
%While ideally it looks like a plausible solution, these approaches have limited practicality because they cannot handle videos of significant length in the fully end-to-end manner.
However, these approaches have limited practicality because they cannot process significant-length videos in a fully end-to-end manner.
When processing long videos, inter-clip association is necessary as the video must be split into multiple clips that the GPU can hold.
Therefore, in order to handle long videos, associating frame- or clip-level predictions through heuristics is an unavoidable process in all previous methods.
%they should split the video in multiple clips that GPU can hold, thus an inter-clip stitching becomes undoubtedly necessary.

%, which again requires hand-crafted algorithms.
In this work, we argue that the processed units (frames, clips, and videos) are only optional, and the fundamental question is rather ``\emph{how to learn the association between separately processed units?}''.
One preceding study, EfficientVIS~\cite{EfficientVIS}, devises a simple solution using the correspondence between \emph{paired} clips.
The key idea is propagating the decoded object queries from the first clip as input to the following clip, by restricting object queries from the following clip to keep unique identities assigned by the first clip.
% The key idea can be summarized into two points: 1) propagating the decoded object queries from the first clip as input to the following clip; \fix{2) restricting object queries from the following clip to keep unique identities assigned by the first clip.}
%\textcolor{red}{that.... We need how they did it.}
%While it shows competitive performance, we observe that it struggles to handle videos with long sequences.
While it gives initial clues to our question, we observe that it still struggle to handle videos with long sequences.
% Our understanding is that since their learning strategy only considers two consecutive clips, the discrepancy between the learning and real-world videos causes the vulnerability.
Our understanding is that the discrepancy between the learning and real-world videos causes the vulnerability since their approach only considers two consecutive clips.

In this paper, we introduce a \underline{\textbf{Gen}}eralized \underline{\textbf{VIS}} framework, namely \textbf{\name{}} (\cref{fig:teaser} (c)), that is designed to \emph{minimize} the gap of  between training and inference by .
% To effectively model temporal characteristics by making multi-clip\footnote{In this paper, we denote \emph{clip} as a generic term covering the scope of single or multiple video frames.} training possible, we introduce a \underline{\textbf{Gen}}eralized \underline{\textbf{VIS}} framework, namely \textbf{\name{}} (\cref{fig:teaser} (c)).
% The main goal of \name{} is to ``\emph{minimize the gap between training and inference}''.
We propose learning strategy that can be plugged in the existing query-based VIS methods to make long-term tracking robust without heuristic object association between units.
We adopt VITA~\cite{VITA} as our clip-level predictor, which learns clip-level queries to represent each object. 
% Our learning strategy can be plugged in the existing query-based VIS methods to make long-term tracking robust without heuristic object association between units.
% In this paper, we adopt VITA~\cite{VITA} as our clip-level predictor, which learns clip-level queries to represent each object. 
% As VITA re-uses frame-level object queries from an pre-trained image detector~\cite{Mask2Former}, it requires less GPU memory during training.  
We can adjust the unit clip length for VITA to create \emph{online} and \emph{semi-online} variants for GenVIS. 
By setting the unit length as one, it become online VIS model that processes a video frame-by-frame. 
By having the unit length larger than one, it runs in a semi-online that processes a video clip-by-clip.  

% is a memory-efficient  has shown that a frame can be precisely parsed by decoding the scene using a number of object queries.
% However, the underlying challenge is the capacity to fit the multiple clips into GPU memory during training time.
% We overcome the issue by adopting VITA~\cite{VITA} as our clip-level predictor, which has shown that a frame can be precisely parsed by decoding the scene using a number of object queries.
% Leveraging such findings, VITA achieves immense reduction in GPU memory by discarding spatio-temporal features and using frame-level queries only to represent an input video.
% By utilizing VITA as our clip-level predictor, a clip can be succinctly represented with a number of clip queries that hold object-centric information.
% \textcolor{red}{therefore, video-level training is possible.}

% In this regard, 
% Here, we set the first condition for general VIS framework: c1) the model flexibly change the range of scope \emph{without} modification.
% In this regard, we first look back on the boundary of existing approaches and take further step to explore a generalized framework for VIS.

%In other words, current architectures also require matching between independent clip-level predictions using post-processing.   
%they miss the underlying continuity of time.
% In this paper, we claim that the units of processing inputs -- frames, clips, and videos -- is only an option, and the fundamental question is rather ``how to seamlessly stitch separately processed units?''.

% In this regard, we first look back on the blurry boundary of approaches and take further step to explore a generalized framework for VIS.
%Our interpretation is that the key is how many frames in a row of videos are employed to understand a video.
%Now, the natural question is, how 
% We observe that, of course, it depends on the purpose and the characteristics of input data.
% For example, if the purpose is to understand complex motion under streaming, prediction with sort-term range is effective while multiple frames may be effective to consider long contexts if the purpose is to understand high-level scenes.
% Here, we set the first condition for general VIS framework: c1) the model flexibly change the range of scope \emph{without} modification.
% In this paper, we denote \emph{clip} as a general term to cover the scope of one or more video frames.

%By loading multiple clips in the training phase, we bridge the gap between learning and real-world, 
% Now capable of making use of multiple clips during training, we propose a better training strategy that resembles real-world videos.
The essence of GenVIS is new training strategy. Our tracking algorithm is inspired by the propagating query paradigm, initially proposed in EfficientVIS~\cite{EfficientVIS}. 
While adopting the key idea, we make two further improvements.
%\textcolor{red}{How EfficientVIS and us do tracking (e.g., using query)?, what is their learning strategy?}
First, we increase the number of clips during training (\emph{i.e., from 2 to 5)} to make the training more similar to realistic long video inference. 
But, this na\"ive extension does not give us meaningful performance boost. 
We find that the bottleneck lies in the prediction-target assignment algorithm in loss computing.
Target assignment proposed in~\cite{EfficientVIS} is not designed to deal with more than two clips; cannot fully reflect various scenarios in long-ranged tracking.
As the second improvement, we introduce new target assignment algorithm that covers newborn objects and objects disappear-and-reappear.
With our learning strategy, we not only improve tracking performance, but also remove heuristics\footnote{\fix{Determine whether a query is classified as background to reinitialize.}} from the inference stage.
That is, our model infers videos in exactly the same way as learned.


% We empirically find that na\"ively extending the number of clips from pairs to multiples (\emph{i.e., 5}) at training time is beneficial to boost performance.
% Narrowing the gap between the learning and real-world by loading multiple clips at training stage, we revisit propagating query paradigm initially discovered in EfficientVIS.
% Under the realistic perspective that continuous clips are endless, our next step is eliminating manually designed heuristics that are vulnerable to domain changes.
% We empirically find that na\"ively extending the number of clips from pairs to multiples (\emph{i.e., 5}) at training time is beneficial to boost performance.
% However, its target assignment algorithm is not designed to deal with multiple clips; cannot fully reflect various tracking scenarios.
% To improve this, we introduce new target label assignment strategy that covers  any clip queries can detect newborn objects or track appeared objects.
% Thanks to this strategy, we not only improve tracking performance, but also remove heuristics from the inference stage.
% That is, our model infers videos in exactly the same way as learned.

To further improve performance by leveraging a sequence of multiple clips, we build a memory that stores previously decoded clip queries.
Specifically, at every cascaded clip queries propagate the next clip, we simply add extra information obtained by readout operation from stacked memory. 
Since our clip queries preserve its ID throughout sequences, we localize the attention on the history of same instance to focus on previous trajectories of unique instance.
As our memory readout is a local attention operation, it is memory efficient and has minimal computational overhead.

%we set the second condition: c2) the model views the scene as a continuous sequence and seamlessly runs rather than \emph{connecting} separate clips.
%From a technical standpoint, the gap between learning and testing stages should be eliminated as much as possible.

% There were several attempts to split a video into multiple clips (\emph{i.e.}, a group of frames) and match independent clip-level mask tracklets using post-processing~\cite{MaskProp, IFC}.
% However, since the algorithm relies on heuristics such as mask IoU of overlapped frames between adjacent clips, it leads to heavy memory consumption.
% Recently, EfficientVIS~\cite{EfficientVIS} proposes correspondence learning for two consecutive non-overlapped clips that supervises \fix{the track queries output from one clip to segment and correspond to the same object instances in the next clip.}
% % These methods effectively devise a solution that not only employs temporal context in the local window but also processes any videos despite the length, they \emph{volatilize} memory of the past because consider only two consecutive clips.
% Although these methods not only utilize temporal contexts in local windows, but also handle all videos regardless of length, they \emph{volatilize} past memories because they only consider two consecutive clips.

% In order to achieve above goals, we propose a \underline{\textbf{Gen}}eralized \underline{\textbf{VIS}} framework, namely \name{}.
%(\cref{fig:teaser} (c)) to effectively understand objects spanning a long time axis.
% Specifically, our method aims to (1) predict tracklets by making use of near context within a short-range clip, (2) seamlessly \emph{splice} tracklets in successive clips, and (3) deploy object-centric history to understand current clip.
% The underlying problem, however, is the capacity to fit the multiple clips into GPU memory during training time.

% To this end, we overcome the issue by adopting VITA~\cite{VITA} as our clip prototype generator, which brings about modeling temporal characteristics by making multi-clip training possible.
% Recent studies~\cite{MinVIS, VITA} has shown that a frame can be precisely parsed by decoding the scene using a number of object queries.
% Leveraging such findings, VITA~\cite{VITA} achieves immense reduction in GPU memory by discarding spatio-temporal features and using frame-level queries only to represent an input video.
% By utilizing VITA as our clip prototype generator, a clip can be succinctly represented with a number of clip queries that hold object-centric information.

Despite the simple and intuitive framework, \name{} achieves state-of-the-art results on the VIS benchmarks without bells and whistles.
Notably, \name{} greatly exceeds the state-of-the-art performance on challenging long and complex video datasets, Occluded VIS and YouTube-VIS 2022.
Importantly, we validate the generalization capability of our method by setting the record under both per-frame and per-clip manner.
In addition to performance, we provide further analysis of training and inference settings that can be utilized for generalized purposes beyond VIS tasks. 
%We summarize the contributions of this paper as follows.
% \begin{itemize}
% \item We provide simple framework GenVIS generalize multiple clips long videos
% \item eliminates heuristic
% \item GenVIS seamlessly unifies per-frame and per-clip video instance segmentation by showing state-of-the-art performance.
% \item memory optional
% \end{itemize}


==> tab/ablation_clip_len.tex <==
\begin{table}
\centering
{
\begin{tabular}{c|ccccc}
\toprule
$N_{f}$  & AP        & AP$_{50}$     & AP$_{75}$     & AR$_{1}$      & AR$_{10}$ \\
\midrule
\midrule
1            & 33.0 & 56.8 & 34.3 & 15.7 & 37.5 \\ 
\textbf{3}   & \textbf{33.4} & \textbf{57.8} & \textbf{34.5} & \textbf{15.7} & \textbf{37.7}  \\
5            & 31.3 & 56.0 & 32.8 & 15.3 & 35.9  \\
7            & 29.7 & 51.4 & 30.7 & 14.6 & 34.0 \\
\bottomrule
\end{tabular}
}
\caption{
%
ablation ovis validation R50 - Number of frames for a clip - 5 clips are used for training.
% 
}
\label{tab:clip_len}
\end{table}

==> tab/ablation_clip_num.tex <==
%%% clip len = 5 & sampling range = {12, 18, 24, 24/30?}
\begin{table}
\centering
{
\begin{tabular}{c|ccccc}
\toprule
$N_{v}$  & AP        & AP$_{50}$     & AP$_{75}$     & AR$_{1}$      & AR$_{10}$ \\
\midrule
\midrule
2            & & & & &  \\
3            & 33.4 & 57.8 & 34.5 & 15.7 & 37.7  \\
7            &  &  & & &  \\
9            &  & &  & &  \\
\bottomrule
\end{tabular}
}
\caption{
%
ablation ovis validation R50 -- Number of clips used for training
% 
}
\label{tab:ovis}
\end{table}

%%% clip len = 5 & sampling range = 24
% \begin{table}
% \centering
% {
% \begin{tabular}{c|ccccc}
% \toprule
% $N_{v}$  & AP        & AP$_{50}$     & AP$_{75}$     & AR$_{1}$      & AR$_{10}$ \\
% \midrule
% \midrule
% 2            & 28.0 & 48.5 & 28.2 & 13.7 & 32.7  \\
% 5            & 30.9 &  &  &  &  \\
% 7            & 30.9 & 53.4 & 32.5 & 15.4 & 35.8 \\
% 9            & 31.0 & 54.2 & 31.7 & 15.5 & 35.8 \\
% \bottomrule
% \end{tabular}
% }
% \caption{
% %
% ablation ovis validation R50 -- Number of clips used for training
% % 
% }
% \label{tab:ovis}
% \end{table}

==> tab/ablation_mems.tex <==
\begin{table}
\centering
{
\begin{tabular}{c|ccccc}
\toprule
 Memory      & AP        & AP$_{50}$     & AP$_{75}$     & AR$_{1}$      & AR$_{10}$ \\
\midrule
\midrule
vanila &&&&\\
 global attn                     & &&&&  \\
 index attn                     & &&&&  \\
\bottomrule
\end{tabular}
}
\caption{
%
ablation ovis validation R50
% 
}
\label{tab:ovis}
\end{table}

==> tab/rebu_small_labels.tex <==
\begin{table}[H]
\centering
\vspace{-3mm}
{
\begin{tabular}{l|ccccc}
\toprule
Training  & AP        & AP$_{50}$     & AP$_{75}$     & AR$_{1}$      & AR$_{10}$ \\
\midrule
Full            & 45.2 & 69.1 & 48.4 & 19.1 & 48.6\\ 
10\%            & 35.5 & 56.2 & 36.0 & 16.8 & 39.3 \\
% 5\%             &  & &  &  &  \\
%1\%             &  &  &  &  &  \\
\bottomrule
\end{tabular}
}
\vspace{-3mm}
% \caption{
% %
% ablation ovis validation R50 - Number of frames for a clip - 5 clips are used for training.
% % 
% }
\label{tab:clip_len}
\end{table}

==> tab/ytvis_2019.tex <==
\begin{table*}
\centering
%\resizebox{\linewidth}{!}
{ %< auto-adjusts font size to fill line
\begin{tabular}{c|l|l|ccccc}
    \toprule
\multicolumn{2}{l|}{Method}                     & Backbone      & AP        & AP$_{50}$ & AP$_{75}$ & AR$_1$    & AR$_{10}$ \\
    \midrule
    \midrule
    \multirow{9}{*}{\rotatebox{90}{Offline}}
    & VisTR~\cite{VisTR}                        & ResNet-50     & 35.6      & 56.8      & 37.0      & 35.2      & 40.2      \\
    & IFC~\cite{IFC}                            & ResNet-50     & 41.2      & 65.1      & 44.6      & 42.3      & 49.6      \\
    & TeViT~\cite{TeViT}                        & MsgShifT      & 46.6      & 71.3      & 51.6      & 44.9      & 54.3      \\
    & SeqFormer~\cite{SeqFormer}                & ResNet-50     & 47.4      & 69.8      & 51.8      & 45.5      & 54.8      \\
    & SeqFormer~\cite{SeqFormer}                & Swin-L        & 59.3      & 82.1      & 66.4      & 51.7      & 64.4      \\
    & Mask2Former-VIS~\cite{Mask2Former-VIS}    & ResNet-50     & 46.4      & 68.0      & 50.0      & -         & -         \\
    & Mask2Former-VIS~\cite{Mask2Former-VIS}    & Swin-L        & 60.4      & 84.4      & 67.0      & -         & -         \\
    & VITA~\cite{VITA}                          & ResNet-50     & 49.8      & 72.6      & 54.5      & 49.4      & 61.0      \\
    & VITA~\cite{VITA}                          & Swin-L        & 63.0      & 86.9      & 67.9      & 56.3      & 68.1      \\
    \midrule
    \multirow{11}{*}{\rotatebox{90}{(Near) Online}}
    & MaskTrack R-CNN~\cite{MaskTrackRCNN}      & ResNet-50     & 30.3      & 51.1      & 32.6      & 31.0      & 35.5      \\
    & CrossVIS~\cite{CrossVIS}                  & ResNet-50     & 36.3      & 56.8      & 38.9      & 35.6      & 40.7      \\
    & PCAN~\cite{PCAN}                          & ResNet-50     & 36.1      & 54.9      & 39.4      & 36.3      & 41.6      \\
    & EfficientVIS~\cite{EfficientVIS}          & ResNet-50     & 37.9      & 59.7      & 43.0      & 40.3      & 46.6      \\
    & VISOLO~\cite{VISOLO}                      & ResNet-50     & 38.6      & 56.3      & 43.7      & 35.7      & 42.5      \\
    & MinVIS~\cite{MinVIS}                      & ResNet-50     & 47.4      & 69.0      & 52.1      & 45.7      & 55.7      \\
    & MinVIS~\cite{MinVIS}                      & Swin-L        & 61.6      & 83.3      & 68.6      & 54.8      & 66.6      \\
    & IDOL~\cite{IDOL}                          & ResNet-50     & 49.5      & 74.0      & 52.9      & 47.7      & 58.7      \\
    & IDOL~\cite{IDOL}                          & Swin-L        & 64.3      & 87.5      & 71.0      & 55.6      & 69.1      \\
    \cmidrule{2-8}
    & Ours                                     & ResNet-50      & 51.2      & 71.8      & 57.2      & 48.9      & 59.2      \\
    & Ours                                     & Swin-L         & & & &      \\
    \bottomrule
    \end{tabular}
} %< \resizebox
\caption{
% 
Comparisons on YouTube-VIS 2019.
% 
}
\label{tab:ytvis2019}
\end{table*}

==> tab/ytvis_2021.tex <==
\begin{table}
\centering
{
\begin{tabular}{l|ccccc}
\toprule
Method                                  & AP        & AP$_{50}$     & AP$_{75}$     & AR$_{1}$      & AR$_{10}$ \\
\midrule
\midrule
% MaskTrack R-CNN~\cite{MaskTrackRCNN}    & 28.6      & 48.9          & 29.6          & 26.5          & 33.8      \\
STMask~\cite{STMask}                    & 31.1      & 50.4          & 33.5          & 26.9          & 35.6      \\
%SipMask~\cite{SipMask}                 & 31.7      & 52.5          & 34.0          & 30.8          & 37.8      \\
%QueryInst-VIS~\cite{QueryInst-VIS}     & 14.7      & 34.7          & 11.6          & 9.0           & 21.2      \\
CrossVIS~\cite{CrossVIS}                & 34.2      & 54.4          & 37.9          & 30.4          & 38.2      \\
IFC~\cite{IFC}                          & 35.2      & 55.9          & 37.7          & 32.6          & 42.9      \\
VISOLO~\cite{VISOLO}                    & 36.9      & 54.7          & 40.2          & 30.6          & 40.9      \\
TeViT$^\dagger$~\cite{TeViT}            & 37.9      & 61.2          & 42.1          & 35.1          & 44.6      \\
SeqFormer~\cite{SeqFormer}              & 40.5      & 62.4          & 43.7          & 36.1          & 48.1      \\
Mask2Former-VIS~\cite{Mask2Former-VIS}  & 40.6      & 60.9          & 41.8          & -             & -         \\
IDOL~\cite{IDOL}                        & 43.9      & 68.0          & 49.6          & 38.0          & 50.9      \\
MinVIS~\cite{MinVIS}                    & 44.2      & 66.0          & 48.1          & 39.2          & 51.7      \\
VITA~\cite{VITA}                        & 45.7      & 67.4          & 49.5          & 40.9          & 53.6      \\
\midrule
% Ours                                    & 47.0      & 67.6          & 51.9          & 39.8          & 53.6      \\
Ours (new)                              & 47.8      & 68.6          & 52.1          & 41.1          & 54.5      \\ % added by JS
\bottomrule
\end{tabular}
}
\caption{
%
youtube vis 2021 validation R50
% 
}
\label{tab:ytvis_2021}
\end{table}
